Declarative Privacy-Preserving Inference Queries

Detecting inference queries running over personal attributes and protecting such queries from leaking individual information requires tremendous effort from practitioners. To tackle this problem, we propose an end-to-end workflow for automating privacy-preserving inference queries including the detection of subqueries that involve AI/ML model inferences on sensitive attributes. Our proposed novel declarative privacy-preserving workflow allows users to specify "what private information to protect" rather than "how to protect". Under the hood, the system automatically chooses privacy-preserving plans and hyper-parameters.

==> Conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

==> Related.tex <==
\section{System Overview}
\label{sec:challenges}
Significant challenges lie in the complexity of identifying the sensitive part of the query to be replaced, the model architecture for replacing the sensitive sub-query, and the hyper-parameters for training the model. It would require a lot of human resources to manually figure out the optimal scheme and configurations for each query. The lack of declarative and automated tooling poses significant challenges for federated data management. To address this problem, we further advocate for a novel privacy-preserving workflow. The workflow uses taint analysis to automatically identify sensitive sub-queries (Sec.~\ref{subsec: taint}). Then, an AutoML model search process will be invoked to efficiently identify the optimal model search architecture (Sec.~\ref{subsec: DNAS}) that would strike a desired balance among privacy budget, utility (i.e., accuracy), and efficiency. The workflow further allows human experts to review and refine the selected plans.

% \eat{
\noindent
\textbf{(1) Privacy Information Specification.}  Users are allowed to label the attributes and tuples to specify private information that needs to be protected. In addition, the view-based access control policies as supported in most relational database management systems (RDBMSs), can also be used as input for the proposed system to understand the privacy requirements of the relations.

\noindent
\textbf{(2) Query Intermediate Representation (IR) and Taint Analysis.}
The queries over federated data silos will be automatically lowered to an IR that enhances relational algebra to efficiently identify sub-queries that involve sensitive attributes or tuples through taint analysis~\cite{clause2007dytan}.

\noindent
\textbf{(3) Privacy-preserving Transformation Enumeration and Recommendation.} The system will automatically enumerate possible privacy-preserving schemes based on the proposed model-query transformation technique. Those schemes can be applied to the sensitive sub-query as a transformation to the IR. A cost-based optimizer will evaluate the computational costs of each candidate (logical) plan and select the optimal plan using dynamic programming. 

\noindent
\textbf{(4) Efficient Model Search based on Transfer Learning and Neural Architecture Search.} Given a query-model transformation request (e.g., as recommended by the cost model), the system will first search for a pre-trained model that can be reused to implement the transformation through transfer learning~\cite{shen2023hugginggpt}. Then, it will search for the adaptive layer(s) ~\cite{houlsby2019parameter,hu2021lora} to be inserted into the pre-trained model to meet the accuracy, privacy, and latency requirements. If there are no existing pre-trained models that match the task, then we use differential neural architecture search (DNAS)~\cite{liu2018darts} to obtain a deep learning architecture and then train the model from scratch.

\noindent
\textbf{(5) Feedback.} Finally, the human can review and modify the selected privacy-preserving mechanism for audit/compliance and optimization purposes. The final query execution latency and accuracy will also be recorded and used to refine the cost model. 

We will demonstrate an end-to-end declarative privacy-preserving workflow for federated queries based on the proposed techniques from the data owner's and the data scientist's perspectives. We will also demonstrate how the proposed framework achieves flexible trade-offs among privacy, accuracy, and efficiency.
% }

%We will first demonstrate the novel privacy-preserving mechanism based on DP-SGD training and query-model transformation. Then, we will demonstrate an end-to-end declarative privacy-preserving workflow for federated data management that follows the aforementioned five steps using various data sharing scenarios that are designed based on real-world use cases in the department of homeland security (DHS), healthcare, and financial industry.

==> Usecase.tex <==
\section{Alzheimer's Patients Monitoring: A Real-World Use Case}
\label{sec:usecase}

\begin{figure*} 
\centering
\includegraphics[width=1\textwidth]{figures/Use-Case.pdf}
\caption{\label{fig:UI} \small Alzheimer's Patients Monitoring Use Case}
\vspace{-10pt}
\end{figure*}

Monitoring Alzheimer's patients in real-world scenarios is crucial due to various reasons that encompass both the well-being of the patient and the efficiency of caregiving. Firstly, continuous monitoring allows for the tracking of behavioral, cognitive, and health-related changes, aiding in better disease management. Safety concerns, such as wandering or confusion episodes common in Alzheimer's patients, are addressed through monitoring, enabling rapid response to emergencies. Moreover, adherence to prescribed medication schedules is ensured, optimizing treatment effectiveness. Real-time data obtained through monitoring facilitates caregivers in offering timely assistance, ultimately enhancing the overall quality of care provided. Early detection of changes or symptoms also enables prompt medical intervention, potentially slowing the progression of the disease. Ultimately, this real-world use case not only aim to provide proactive care but also strive to maintain a higher quality of life for Alzheimer's patients while supporting their caregivers in the caregiving process. The query processing for Alzheimer's Patients Monitoring real-world use case is illustrated in Figure 4. This particular use case demonstrates the practical application of the proposed framework through the integration of privacy-preserving technique. 

The workflow designed for monitoring Alzheimer's patients unfolds across several key steps, offering a structured approach to its implementation: 

\begin{itemize}
    \item \textbf{Labeled Sensitive Information within Datasets}: 
In the realm of elderly care, enabling patients to share sensitive information with the care organization involves a process where individuals actively label their data points considered sensitive within the dataset. This approach hinges on granting patients agency and control over their information by offering various avenues for explicit consent. Patients are empowered to selectively mark specific data elements or categories they deem sensitive, either through customizable forms, digital interfaces with privacy settings, or direct communication. Educating and engaging patients in conversations about what they perceive as sensitive data ensures a more personalized and respectful approach to data sharing. The Figure 4 shows that the patient's data is annotated as private, which is directly specified by the patients or extracted from view-based access control policy specified by the patients. For instance, personal information such as the name and age of an Alzheimer's patient, along with their vital health statistics (e.g., John, 67 years old, blood pressure: 130/89), is considered sensitive. 
    \item \textbf{Request for Query and Taint Analysis}: 
In the following stage of the process, when a nurse seeks to retrieve specific MRI scan images for a patient at Elderly care-1, this action triggers a sophisticated query transformation. This transformation takes place within a graph-based Information Retrieval (IR) system, employing a nested relational algebra framework. Within this framework, nodes represent different relational operators used in database queries, while edges denote datasets comprising various types of information, such as image files, videos, or textual documents.

What makes this system particularly robust is its ability to track the flow of sensitive information, often referred to as "taint." As the query progresses through the system's structure, any sources or elements of data identified as potentially sensitive, such as private medical information, are marked or "tainted." This taint is then propagated through the structure, effectively tagging any sub-queries or operations that access this sensitive data. This meticulous process aids in identifying and isolating specific queries or segments that touch upon private information, ensuring a higher level of security and privacy within the system.
    \item \textbf{Recommendations with Privacy Preservation}: Our proposed privacy-preserving method, rooted in learning-based query-model transformation, is versatile, suitable for various query types characterized by machine learning or deep learning models capturing their input and output parameters. For instance, consider a query like SELECT MRI\_Images FROM Central\_Hospital\_Organization WHERE Nurse\_Location = 'Elderly Care-1' AND Alzheimer\_Patient\_Name = 'Patient Name' AND Alzheimer\_Patient\_Age = 'Patient Age'. This query can be modeled as a mapping function ('Patient Name', 'Patient Age') that predicts the MRI\_Images. By leveraging these query-model transformations, we move away from sharing raw data and instead share the trained model, significantly enhancing privacy measures.
    \item \textbf{Pre-Trained Model Search}: At the central hospital organization, data regarding visits and health checkups of Alzheimer's patients, including MRI scans, is securely stored. When a nurse submits a query to access a patient's MRI scans, they utilize a pre-trained model specifically designed for this purpose. These pre-trained models are initially trained using DP-SGD, ensuring enhanced privacy during the training process. Leveraging these pre-trained models contributes to achieving high accuracy while minimizing costs. Within this framework, multiple models exist for handling the same query. The proposed system employs a privacy-preserving cost-based optimizer to select the most optimal scheme among these models. If the desired model isn't available as a pre-trained option, the system initiates the training process from scratch, ensuring that required models are available for query handling. This adaptive approach ensures both accuracy and privacy, either through pre-trained models or by dynamically training models when necessary.
    \item \textbf{Feedback}: At the last stage, the nurse is able to get access the patient's MRI scan images without sharing the data by using our proposed framework. For the feedback, a human reviewer can assess and adjust the chosen privacy-protection method for auditing, compliance, and optimization objectives. This evaluation considers the recorded final query execution time and accuracy, contributing to the refinement of the cost model.

We intend to exhibit a comprehensive privacy-preserving workflow for federated queries, showcasing our suggested methods from the viewpoints of both data owners and data scientists. This demonstration aims to illustrate how our framework facilitates adaptable compromises between privacy, accuracy, and efficiency.
\end{itemize}



